An Atemporal Model of Physical Complexity

We present the finite first-order theory (FFOT) machine, which provides an atemporal description of computation. We then develop a concept of complexity for the FFOT machine, and prove that the class of problems decidable by a FFOT machine with polynomial resources is NP intersect co-NP.

==> eptcsdata.tex <==
\providecommand{\firstpage}{39}
\providecommand{\publicationstatus}{M. Cuffaro and P. Papayannopoulos (Eds.): 9th International\\ Workshop on Physics and Computation (PC 2018) \\
EPTCS 273, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.273.4}{10.4204/EPTCS.273.4}}

